VDC: Versatile Data Cleanser based on Visual-Linguistic Inconsistency by Multimodal Large Language Models

The role of data in building AI systems has recently been emphasized by the emerging concept of data-centric AI. Unfortunately, in the real-world, datasets may contain dirty samples, such as poisoned samples from backdoor attack, noisy labels in crowdsourcing, and even hybrids of them. The presence of such dirty samples makes the DNNs vunerable and unreliable.Hence, it is critical to detect dirty samples to improve the quality and realiability of dataset. Existing detectors only focus on detecting poisoned samples or noisy labels, that are often prone to weak generalization when dealing with dirty samples from other domains.In this paper, we find a commonality of various dirty samples is visual-linguistic inconsistency between images and associated labels. To capture the semantic inconsistency between modalities, we propose versatile data cleanser (VDC) leveraging the surpassing capabilities of multimodal large language models (MLLM) in cross-modal alignment and reasoning.It consists of three consecutive modules: the visual question generation module to generate insightful questions about the image; the visual question answering module to acquire the semantics of the visual content by answering the questions with MLLM; followed by the visual answer evaluation module to evaluate the inconsistency.Extensive experiments demonstrate its superior performance and generalization to various categories and types of dirty samples. The code is available at \url{https://github.com/zihao-ai/vdc}.

==> content/intro.tex <==

The emerging concept of data-centric AI (DCAI) highlights the pivotal role of data in constructing advanced AI systems~\cite{zha2023data}. The quality and reliability of data are crucial factors influencing model performance. Nevertheless, in the real world, dataset can be susceptible to undesirable flaws~\cite{whang2023data}. 
% For instance, these imperfections may result from the \textbf{dirty samples} within the datasets.

For instance, \textbf{dirty samples} may be introduced into the datasets intentionally or unintentionally in \cref{fig:example}.
In this paper, we comprehensively examine three categories of dirty samples as follows:\\
\textbf{Category \Rmnum{1}: Poisoned Samples.} In the context of backdoor attack, malicious attackers intentionally manipulate partical clean samples by embedding triggers and changing the ground-truth labels to target labels, thereby generating poisoned samples. Deep neural networks (DNNs) trained on the dataset with such poisoned samples will be injected with backdoor, \ie predict any poisoned sample as the target label during the inference stage, while maintain accuracy on the clean samples.
\\
\textbf{Category \Rmnum{2}: Noisy Labels.} In scenarios of crowdsourcing or web crawling, human annotators or automatic annotation robots may make mistakes accidentally, resulting in the presence of dirty samples with corrupted labels. Training DNNs using the dataset with such noisy labels will significantly degrade the overall performance.
\\
\textbf{Category \Rmnum{3}: Hybrid Dirty Samples.} An even more critical concern arises when the attackers poison datasets that initially contain noisy labels. In this case, the datasets comprise both poisoned samples and noisy labels. Models trained on such datasets will encounter both malicious backdoor attack and performance degradation simultaneously.

\begin{figure}[h]
\centering 
\includegraphics[width=0.8\textwidth]{figs/example.png}
\captionsetup{font=small}
\caption{An example of clean sample/noise label/poisoned sample} 
\label{fig:example} 
\end{figure}

The presence of the above dirty samples makes the DNNs vulnerable and unreliable.
To enhance the robustness and performance of DNNs, the detection of dirty samples is crucial in the lifecycle of DCAI. 
Recent research have been proposed on the noisy label detection \cite{cl,bhn} or poisoned sample detection \cite{spectre,ct} respectively. 
However, they frequently exhibit limitations in terms of generalization:
\textbf{1). Inconsistent generalization across different categories of dirty samples.} We find that detectors designed for detecting poisoned samples are ineffective when applied to datasets with noisy labels, and vice versa. Moreover, both types of detectors prove inadequate for hybrid dirty samples.
\textbf{2). Inconsistent generalization across different types of dirty samples in the same category.}
For noisy label detection, research has shown that symmetric noisy labels are more readily detectable than asymmetric ones~\cite{cores}. Likewise, for poisoned sample detection, sensitivity to various triggers has been demonstrated in ~\cite{backdoorbench}. 
Therefore, developing a universal framework capable of detecting multiple types of dirty samples concurrently, including noisy labels and poisoned samples, is an urgent challenge for DCAI.

We want to use a notable commonality of noisy labels and poisoned samples lies in \textbf{visual-linguistic inconsistency} between visual contents and associated labels, \ie the semantics of visual modality and that of language modality of label do not match, even when the poisoned samples are embedded with triggers.


% Various studies \cite{blosser1991ask,misra2018learning,zhu2023chatgpt} have shown that the ability to ask insightful questions is a sign of intelligence, which plays a vital role in expanding our understanding of the world. 
% Inspired by this, in this paper, we propose \textbf{V}ersatile \textbf{D}ata \textbf{C}leanser (VDC), which is a universal detection framework for any type of dirty samples. It works by asking visual questions to acquire knowledge from images to determine whether the image and label match. 
% \textit{What questions to ask? How to answer the questions? How to evaluate the answers?} are three key points in the VDC.
% Considering the remarkable advancements in visual and linguistic comprehension and reasoning demonstrated by Large Language Models (LLM)~\cite{zhao2023survey} and Multimodal Large Language Models (MLLM)~\cite{yin2023survey}, we harness ChatGPT~\cite{OpenAI} as a professional questioner and evaluator while employing InstrcutBLIP~\cite{instructblip} as a question answer within our framework.

% In detail, as illustrated in \Cref{fig:framework}, VDC consists of three modules. 
% First, the \textbf{Visual Question Generation module}  creates insightful visual questions based on provided labels, including manually designed general questions to extract a holistic understanding of the image, alongside label-specific questions automatically generated by ChatGPT to acquire localized knowledge, encompassing label-related common sense features, attributes, functions, geographical location, history and culture and \etc.
% Then, \textbf{Visual Question Answering module} is responsible for answering these questions based on the image by utilizing MLLM.
% Afterward, \textbf{Visual Question Evaluation module}  in charge of evaluating the correctness of MLLM's responses, employing ChatGPT in conjunction with string matching techniques.
% Finally, a vote-based ensemble aggregates all questions and answers to determine whether the input is a dirty sample. Extensive experiments show that VDC exhibits superior performance in both poisoned sample detection and noisy label detection. Furthermore, VDC maintains its effectiveness even when dataset contains the mixture of poisoned samples and noisy labels.



% Recently, Large Language Models (LLM) have made remarkable progress towards natural language understanding and generation~\cite{ouyang2022training,llama2}. Multimodal Large Language Models (MLLM) ~\cite{palme,blip2} further empower LLM with visual reasoning by introducing multiple modalities into LLM through instruction tuning, which shows its surprising capabilities of solving a wide-range of visual-language tasks (\eg visual question answering (VQA), captioning, OCR-free math reasoning).
% MLLM and LLM have become a potential pathway to achieving artificial general intelligence~\cite{bubeck2023sparks}. 

% Motivated by the visual and semantic understanding and reasoning abilities of MLLM and LLM, in this paper, to improve the quality and of reliability of dataset, we propose a \textbf{V}ersatile \textbf{D}ata \textbf{C}leanser (VDC) to detect mislabeled dirty samples based on MLLM and LLM. The framework are shown in Figure \ref{fig:framework}. Specifically, the data cleanser generation two kinds of visual questions based on the given label, where manually designed general questions are used to extract natural language descriptions about the image, while label-specific questions are automatically generated by LLM, involving label-related attributes, characteristic, functions, \etc. For all labels, the general questions remain the same, while the label-specific questions various cross the labels. The expected answer of general questions is the given label and that of label-specific questions is \textit{`yes'}. Then the MLLM are used to answer these visual questions based on the image. The output are evaluated with string matching or LLM through designed prompt. We adopt LLM (GPT-3.5 in the experiments) coupled with string matching as a evaluator to judge if the output and expected answer are match. Finally, the results of all visual questions are aggregated to voted whether the input is a dirty sample. 









